It is Not as Good as You Think! Evaluating Simultaneous Machine Translation on Interpretation Data

Most existing simultaneous machine translation (SiMT) systems are trained and evaluated on offline translation corpora. We argue that SiMT systems should be trained and tested on real interpretation data. To illustrate this argument, we propose an interpretation test set and conduct a realistic evaluation of SiMT trained on offline translations. Our results, on our test set along with 3 existing smaller scale language pairs, highlight the difference of up-to 13.83 BLEU score when SiMT models are evaluated on translation vs interpretation data. In the absence of interpretation training data, we propose a translation-to-interpretation (T2I) style transfer method which allows converting existing offline translations into interpretation-style data, leading to up-to 2.8 BLEU improvement. However, the evaluation gap remains notable, calling for constructing large-scale interpretation corpora better suited for evaluating and developing SiMT systems.

==> sections/corpus_building.tex <==
\section{Building the Simultaneous Speech Translation Corpus}
\label{sec:corpus_building}
%\input{tables/example_dialogues}
\begin{comment}
\philip{This section contains too much text and hard to digest. Basically what we need is a figure, depicting the overall process of corpus building. We have to move specific processing steps and details to appendix. This section should contains just high level idea of building the parallel corpus from the website.}
\end{comment}

In this section, we  will  describe  the  process  of collecting genuine data from Europarl and creating a dataset which mirrors real-life scenarios. We will then present a test set which is annotated by bilingual annotators, ensuring the genuineness of our experimental results and analysis.


\textbf{Collection} We crawled debate data from European Parliament Plenary which provides SI data for debates. Each crawled data points consists of a trio: transcriptions of speeches in the source language, post-edited offline translations and simultaneous interpretations in the audio form that are then transcribed with Google Speech API. In total, we obtain 5,239 trios (we call them dialogues in this work). Details of the crawling and transcription process are provided in Appendix. Our focus is German-English, but the process is applicable to any other language pair. Table \ref{tab:example} is one example of the dialogues.  

\textbf{Filtering}
To build a dataset with high-quality, we adopted a series of sophisticated automatic and manual preprocessing steps to clean and filter dialogues. We removed dialogues whose 1) source language was non-German; 2) texts are too short; 3) contents were non-essential, determined by pre-defined signals; 4) source transcriptions and translations had different number of sentences. Next, we manually deleted non-essential contents. These steps yielded a total number of 987 dialogues.  

\textbf{Alignment}
Each trio had aligned source transcriptions (German) and post-edited translations (English) and we needed to align transcriptions (English) of live interpretation with the source transcriptions. To do this, we used post-edited translations as mediums that we assigned the English transcriptions to them, as we believe it is easier to align sentences in the same language. The translations in each pair contained several "long" sentences, each of which may have more than one sentence, and thus we call the "long" sentences as super-sentences. Next, we segmented the English transcriptions into smaller chunks, and aligned and re-joint chunks to above super-sentences with dynamic programming (see details in Appendix). It is essential to re-join the chunks considering that in realistic SI scenarios, interpreters often break a long and formal source sentence into multiple smaller pieces. Above process gave us 3,683 data points. After that, we tried to segment super-sentences with almost identical steps, but the resulting pairs were rather noised. This was expected, as human interpreting performance remains suboptimal due to human limited working memory that interpreters may miss or misinterpret information. 

\textbf{Annotation}
It is essential to have realistic SI dataset for any future SiMT systems testing, so we employed a bilingual German-English speaker to annotate a subset of the above aligned dataset. This yielded a test set with a size of 1,090, consisting of trios of \textit{<source, translation, interpretation>}. Details of annotation instructions and quality control procedures are given in Appendix.  




==> sections/corpus_scaling.tex <==
\section{Data Augmentation Approaches for Building Training Data}
\label{sec:corpus_scaling}

Adaptation can be done based on the following techniques together with out-of-domain data:
\begin{itemize}
    \item D1: super-sentence-level pairs obtained from the ASR post-processing. 
   % \item D2: noisy-aligned short sequence pairs obtained from the segmentation algorithm in the previous section. 
    \item D2: crawled normalized monolingual ASR segments from the target side.  
    %\item D3: style-transferred interpreting sequences paired with source sequences.
\end{itemize}
For D2, we use a data argumentation approach with back translation. Specifically, for each target language  sequence $y$ in the target domain, we back-translate it to the source language $\hat{x}$, and then use the pair $(\hat{x},y)$ to adapt the model to the target domain. The back-translation model can be trained on paired out-of-domain data. 

We employ the following approaches to train MT systems with D1 and D2: (i) Pre-train Fine-tune (PTFT): we  train a SiMT model on the source domain and then further fine-tune it on the target domain data; (ii) Mixture (Mix): we train the model with both source domain data and target-domain data from scratch. 
%\item adversarial: We can train one SimNMT model for both source and the target domains, with an adversarial loss to fool a domain classifier. 



==> tables/dataset_statistics.tex <==
\begin{table}[t]
\small
    \centering
    \scalebox{0.8}{
    \begin{tabular}{ l  l l l  }
    \toprule
    Datasets & train & dev & test \\
    \midrule
    % IWSLT &  191,751/887/6,996 \\

    % EUROPARL(fr-en) & \\
    % EUROPARL(pl-en) &  \\
    % EUROPARL(it-en) & \\
    \cmss{Raw-Inter (filtered)} & 217622 (120114) & 1000 & - \\
    %Mono-Inter (filtered) & 120,114/-/- \\
    %Long-Noised & 2,983/300/-  \\
    % D2 & 71,431/500/- \\
    \cmss{Clean-Inter (filtered)} & 10021 (4240) & - & - \\
    %Short-Noised (filtered) & 4,240/-/- \\
    %Translation/Interpretation test & - & - & 1051$^*$ \\
    %Interpretation test & -/-/1,051$^*$ \\
    %Europarl/Europarl\_T2I & 1666904 & 3587 & 5075$^*$ \\
    EPTIC & 1636 & - & - \\
    %Inter-Europarl& 1,666,904/3,587/5,075$^*$\\
    \bottomrule
    \end{tabular}}
    \caption{Dataset statistics. $^*$: Data points that are heavily overlapped with any training data are removed.\ehsan{this table now seems insignificant and we can merge this into text}}
    \label{tab:data}
    \vspace{-2.5mm}
\end{table}

==> tables/full_europarl_annotated.tex <==
\begin{comment}


\begin{table*}
\centering
\small
  \scalebox{0.75}
  {
  \begin{tabular}{l|cccc|cccc|cccc|cccc}
    \toprule
    &  \multicolumn{4}{c}{EUROPARL}  & \multicolumn{4}{c}{Translation Test} & \multicolumn{4}{c}{Translation-suboptimal Test} & \multicolumn{4}{c}{Interpretation Test}\\
    Model & AP & AL & Bleu & Meteor & AP & AL& Bleu & Meteor & AP & AL& Bleu & Meteor & AP & AL& Bleu & Meteor\\
    \midrule
    % \textit{wait-2}\\
    % \addlinespace[0.3em]
    % Europarl  & 0.57& 2.03&20.90 &0.58 &2.19 &22.86 &0.58 &2.19 &11.24  \\
    % D1 + Europarl (PTFT) &0.57 &2.04 &19.91 & 0.59& 2.23&21.12 &0.59 & 2.22& 10.67 \\
    % D2 + Europarl (PTFT)  & 0.57& 1.94& 18.20& 0.58& 2.07& 19.15& 0.58&2.07 &11.30 \\
    % %D3 + Europarl (PTFT) & & & & & & & & & \\
    % D1 + D2 + Europarl (PTFT) &0.57 &1.95 &18.10 & 0.58& 2.11&18.93 & 0.58& 2.11&11.35 \\ 
    % %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    % D2  &0.58 &2.13 &8.70 & 0.59& 2.24&10.48 & 0.59&2.24 &9.45 \\
    % D1 + Europarl (MIX) & 0.57& 1.98& 17.00& 0.58& 2.14&18.11 &0.58 & 2.14& 9.52  \\
    % D2 + Europarl (MIX) & 0.57&1.93 & 17.09& 0.58& 2.06&18.32 &0.58 &2.06 &11.08 \\
    % %D3 + Europarl (MIX) & & & & & & & & & \\
    % D1 + D2 + Europarl (MIX) &0.57 &1.90 & 15.69& 0.58&2.06 &16.70 & 0.58& 2.06& 10.62 \\ 
    
    % %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    % \hline
    \textit{wait-3} \\
    \addlinespace[0.3em]
    Europarl  &0.60 & 2.66&21.52& & 0.61& 2.84&22.82 && & & &&0.61 &2.84 &11.38 & \\
    Europarl-suboptimal \\
    D1 + Europarl (PTFT) &0.60 &2.70 & 22.07&& 0.61&2.93 &23.16& & & & &&0.61 &2.93 &11.52& \\
    D2 + Europarl (PTFT) &0.59 &2.58 &19.64 && 0.61&2.77 &20.75& & & & &&0.61 &2.77 &11.94& \\
    %D3 + Europarl (PTFT) & & & & & & & & & \\
    D1 + D2 + Europarl (PTFT) &0.59 &2.57 &19.38 &&0.61 &2.71 &20.18& & & & & &0.61& 2.71& 11.58 &\\ 
    %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    D2  & 0.61& 2.78& 9.39&&0.62 & 2.90&11.07& & & & &&0.62 &2.90 &9.63& \\
    D1 + Europarl (MIX) & 0.59&2.71 &22.29& &0.62 &2.95 &23.21& & & & &&0.61 &2.95 &11.79& \\
    D2 + Europarl (MIX) & 0.59& 2.56&18.36 &&0.61 &2.72 &19.72 && & & &&0.61 &2.72 &11.49& \\
    %D3 + Europarl (MIX) & & & & & & & & & \\
    D1 + D2 + Europarl (MIX) &0.59 &2.59 &17.61& &0.61&2.78 &18.89 && & & &&0.61 &2.78 & 11.10& \\ 
    %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    \hline
    \textit{wait-4} \\
    Europarl  & 0.62& 3.40& \textbf{23.59} &&0.64 &3.63 & \textbf{24.42}& & & & &&0.64 &3.63 &11.90&  \\
    Europarl-suboptimal \\
    D1 + Europarl (PTFT) & 0.62& 3.46&23.05 &&0.64 &3.66 &23.40& & & & & &0.64& 3.66&11.65& \\
    D2 + Europarl (PTFT) &0.62 &3.30 &20.85& &0.64 &3.51 & 22.06 && & & & &0.64& 3.51& \textbf{12.79}& \\
    %D3 + Europarl (PTFT) & & & & & & & & & \\
    D1 + D2 + Europarl (PTFT) & 0.62& 3.32& 21.02&&0.64 &3.52 &21.66 && & & & &0.64& 3.52&12.47& \\ 
    %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    D2  & 0.63& 3.49&10.00 &&0.65 &3.72 &11.68 && & & &&0.65 &3.72 &10.27 &\\
    D1 + Europarl (MIX) & 0.62 &3.27 &19.32 &&0.64 &3.49 &20.30& & & & &&0.64 &3.49 &10.34& \\
    D2 + Europarl (MIX) & 0.62& 3.29& 19.00&&0.64 &3.51 &19.62 && & & &&0.64 &3.51 &11.80& \\
    %D3 + Europarl (MIX) & & & & & & & & & \\
    D1 + D2 + Europarl (MIX) & 0.62& 3.21&18.22& &0.64 &3.39 &18.70 && & & &&0.64 &3.39 &11.31 &\\ 
    %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    \hline
    \textit{Coupled Policy}\\
    \addlinespace[0.3em]
    Europarl  &0.65 &3.75 & \textbf{23.09} &&0.67 &4.22 &\textbf{23.63} && & & &&0.67 &4.22 &11.39&  \\
    Europarl-suboptimal \\
    D1 + Europarl (PTFT) & 0.75 & 5.54 & 18.56 && 0.75& 4.85&19.55& & & & & &0.75 &4.85 &9.76 &\\
    D2 + Europarl (PTFT) & 0.63 & 3.07& 20.97&& 0.64&3.13 &20.64 && & & & &0.64& 3.13&\textbf{12.18}& \\
    %D3 + Europarl (PTFT) & & & & & & & & & \\
    D1 + D2 + Europarl (PTFT)  &0.95 &16.89 &13.59 && 0.95 & 13.70 &14.30 && & & & &0.95 & 13.70 & 8.49 &\\ 
    %D1 + D2 + D3 + Europarl (PTFT) & & & & & & & & & \\ 
    D2  & 0.62& 2.15& 10.60&& 0.64& 2.72& 12.00&& & & && 0.64 &2.72 &10.42 &\\
    D1 + Europarl (MIX) &0.67 & 5.00 &18.31& &0.69 & 5.05& 18.31 & & & & & &0.69&5.05 &9.49 &\\
    D2 + Europarl (MIX) &0.63 &2.69 & 19.02&& 0.66& 3.34& 18.89 && & & & &0.66 & 3.34& 11.26&\\
    %D3 + Europarl (MIX) & & & & & & & & & \\
    D1 + D2 + Europarl (MIX) &0.63 & 2.64& 17.91&& 0.65&3.10 &18.34 &&& & & & 0.64& 3.10& 10.92&\\ 
    %D1 + D2 + D3 + Europarl (MIX) & & & & & & & & & \\ 
    \bottomrule
  \end{tabular}
  }
  \caption{Europarl: Out-of-domain data from EUROPARL. 
  PTFT: Pre-train Fine-tune domain adaptation. MIX: Mixture domain adaptation. \textbf{Bold}: The best results.
  \philip{We need to redo most of the experiment. First: (1) it is better to use EUROPARL original dataset for pretrain. This dataset is more comparable to our dataset. (2) We have to compare translating from $x$ to $y_i$ vs $x$ to $y_o$ and shows that it is better for us to translate from $x$ to $y_i$} }
  %ADV: Adversarial domain adaptation (not the priority for now). BKT: domain adaptation with back-translation.}
  \label{tab:results}
\end{table*}
\end{comment}
% \begin{table*}
% \centering
% \small
%   \scalebox{0.85}
%   {
%   \begin{tabular}{l|ccc|ccc}
%     \toprule
%     &  \multicolumn{3}{c}{IWSLT}  & \multicolumn{3}{c}{Annotated Test}\\
%     Model & AP & AL  & Bleu  & AP & AL& Bleu\\
%     \midrule
%     \textit{wait-2}\\
%     \addlinespace[0.3em]
%     Europarl & 0.61 & 2.26  & 20.00 & 0.58 & 2.14  & 7.31 \\
%     D1 + Europarl (PTFT) & 0.61 & 2.27  & 19.93  & 0.57 & 2.11  & 6.93 \\
%     D2 + Europarl (PTFT) & 0.60 & 2.16  & 19.42  & 0.57 & 1.93  & 7.90 \\
%     D1 + D2 + Europarl (PTFT) & 0.61 & 2.19 & 19.80 & 0.57 & 1.91 & 8.55 \\ 
%     D2 & 0.61 & 2.24 & 5.03  & 0.57 & 1.97 & 5.24 \\
%     D1 + Europarl (MIX) & 0.61 & 2.37 & 18.08 & 0.58 & 2.29 & 5.87 \\
%     D2 + Europarl (MIX) & 0.61 & 2.21 & 17.56 & 0.57  & 1.91 & 7.70 \\
%     D1 + D2 + Europarl (MIX) & 0.62 & 2.66 & 14.64 & 0.58 & 2.36 & 6.28 \\ 
%     \hline
%     \textit{wait-3} \\
%     \addlinespace[0.3em]
%     Europarl & 0.65 & 2.95 & 21.26 & 0.60 & 2.78 & 7.52 \\
%     D1 + Europarl (PTFT) & 0.64 &2.94 & \textbf{22.03} & 0.60 & 2.71& 7.38  \\
%     D2 + Europarl (PTFT) & 0.64 & 2.94 & 21.41 & 0.60 & 2.74 & \textbf{9.30} \\
%     D1 + D2 + Europarl (PTFT) & 0.64 & 2.90 & 20.99 & 0.59 & 2.62 & 9.02 \\ 
%     D2 & 0.64 & 2.85 & 6.04 & 0.60 & 2.54& 6.16\\
%     D1 + Europarl (MIX) & 0.64 & 2.93 & 17.33 & 0.60& 2.80 & 5.95  \\
%     D2 + Europarl (MIX) & 0.64 & 2.93 & 20.10 & 0.60 & 2.59 & 8.70 \\
%     D1 + D2 + Europarl (MIX) & 0.65 & 3.27 & 15.94 & 0.61 & 2.94 & 7.06 \\ 
%     \hline
%     \textit{wait-4} \\
%     Europarl & 0.68 & 3.73 & 23.21 & 0.63 & 3.46 & 7.88  \\
%     D1 + Europarl (PTFT) & 0.68 & 3.75 & 22.52 & 0.63 & 3.42 & 7.63  \\
%     D2 + Europarl (PTFT) & 0.68 & 3.64 & 22.17 & 0.62 & 3.28 & 9.55  \\
%     D1 + D2 + Europarl (PTFT) & 0.68 & 3.65 & 22.11 & 0.62 & 3.25 & 9.20  \\ 
%     D2 & 0.68 & 3.65 & 6.28 & 0.62 & 3.31& 6.52 \\
%     D1 + Europarl (MIX) & 0.68 & 3.75& 18.82& 0.63& 3.57& 6.00  \\
%     D2 + Europarl (MIX) & 0.68 & 3.69 & 21.22 & 0.62 & 3.20 & 9.31 \\
%     D1 + D2 + Europarl (MIX) & 0.68 & 3.79 & 19.29 & 0.62 & 3.32 & 8.44 \\ 
%     \hline
%     \textit{Coupled Policy}\\
%     \addlinespace[0.3em]
%     Europarl & 0.62 & 2.39  & 21.50 & 0.62 & 2.71  & 7.46 \\
%     D1 + Europarl (PTFT) & 0.63 & 2.44  & 21.57 & 0.63 & 2.81  & 7.68 \\
%     D2 + Europarl (PTFT) & 0.63 & 2.45 & \textbf{21.81} & 0.62 & 2.68  & 9.14 \\ 
%     D1 + D2 + Europarl (PTFT) & 0.63 & 2.44 & 20.75 & 0.61 & 2.54 & 9.49 \\
%     D2 & 0.65 & 2.99  & 7.03 & 0.64 & 3.48  & 6.53 \\
%     D1 + Europarl (MIX) & 0.63 & 2.63 & 18.02 & 0.62 & 2.85 & 5.70 \\
%     D2 + Europarl (MIX) & 0.63 & 2.37 & 19.80 & 0.63 & 2.76 & \textbf{9.68} \\
%     D1 + D2 + Europarl (MIX) & 0.62 & 2.42 & 20.04 & 0.61 & 2.66 & 9.10\\ 
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Europarl: Out-of-domain data from IWSLT 2016. 
%   PTFT: Pre-train Fine-tune domain adaptation. MIX: Mixture domain adaptation. \textbf{Bold}: The best results.
%   \philip{We need to redo most of the experiment. First: (1) it is better to use EUROPARL original dataset for pretrain. This dataset is more comparable to our dataset. (2) We have to compare translating from $x$ to $y_i$ vs $x$ to $y_o$ and shows that it is better for us to translate from $x$ to $y_i$}}
%   %ADV: Adversarial domain adaptation (not the priority for now). BKT: domain adaptation with back-translation.}
%   \label{tab:results}
% \end{table*}

==> tables/strategy.tex <==
\begin{table*}
\centering
\small
  \scalebox{0.85}
  {
  \begin{tabular}{l|p{5cm}|p{5cm}|p{5cm}}
    \toprule
    \textbf{Strategy} & \textbf{Source} & \textbf{Interpreted Text}  & \textbf{Translated Text}  \\
    \midrule
    Segment \textcolor{orange}{$\vert\vert\vert$} & Man kann darüber streiten, ob die Modellpolitik der europäischen Hersteller, insbesondere der deutschen, verantwortlich war für die Krise, die wir jetzt haben. & You can argue whether the model policy of the European manufacturers in particular. \textcolor{orange}{$\vert\vert\vert$} The German one was responsibility for the crisis that we have. & People can argue about whether the choice of models produced by European manufacturers, especially the German manufacturers, was responsible for the crisis we are now in. \\
    \textcolor{DarkBlue}{Generalize} & Herr Präsident, meine Damen und Herren! Sicherheit ist ein hohes Gut. & President ladies and gentlemen safety is \textcolor{DarkBlue}{very important}. & Mr President, ladies and gentlemen, safety is \textcolor{DarkBlue}{a sacred thing}. \\
    \greenuline{Summarize}, \textcolor{DarkGreen}{(Omit)} & Ich werde an diesem Punkt darauf verzichten, einen Kommentar zur Ernsthaftigkeit dieser Argumentationsweise abzugeben.& I'm not going to comment on \greenuline{that agreement}. & \textcolor{DarkGreen}{(At this point,)} I will refrain from commenting on \greenuline{the seriousness of this line of argument}.  \\
    \redwave{Passive} & Die Frage der Exterritorialität wäre auch zu lösen. & The extraterritorial question also \redwave{needs to be resolved}. & We \redwave{must also resolve} the question of extraterritoriality. \\
    \bottomrule
  \end{tabular}
  }
  \caption{Examples of strategies exhibited in interpreted texts, in comparison with corresponding translated texts.}
  \label{tab:strategies}
\end{table*}

